A search for pair-produced resonances in four-jet final states at $\sqrt{s}$ =13 TeV with the ATLAS detector

A search for massive coloured resonances which are pair-produced and decay into two jets is presented. The analysis uses 36.7 fb$^{-1}$ of $\sqrt{s}=$ 13 TeV pp collision data recorded by the ATLAS experiment at the LHC in 2015 and 2016. No significant deviation from the background prediction is observed. Results are interpreted in a SUSY simplified model where the lightest supersymmetric particle is the top squark, $\tilde{t}$, which decays promptly into two quarks through $R$-parity-violating couplings. Top squarks with masses in the range 100 GeV < $m_{\tilde{t}}$ < 410 GeV are excluded at 95% confidence level. If the decay is into a $b$-quark and a light quark, a dedicated selection requiring two $b$-tags is used to exclude masses in the ranges 100 GeV < $m_{\tilde{t}}$ < 470 GeV and 480 GeV < $m_{\tilde{t}}$ < 610 GeV. Additional limits are set on the pair-production of massive colour-octet resonances.

==> Paper2017/limits.tex <==
\section{Limits}\label{sec:limits}
In the absence of a statistically significant excess in data, exclusion limits can be derived on the signal models of interest.
A profile likelihood ratio combining Poisson probabilities for signal and background is computed
to determine the 95\% CL for compatibility of the data with the signal-plus-background hypothesis (CL$_{s+b}$) \cite{Cowan:2010js}.
A similar calculation is performed for the background-only hypothesis (CL$_b$).
From the ratio of these two quantities, the confidence level for the presence of a signal (CL$_s$ ) is determined \cite{Read:2002hq}.  
Systematic uncertainties are treated as nuisance parameters and are assumed to follow Gaussian distributions. 
The results are evaluated using pseudo-experiments.
This procedure is implemented using a software framework for statistical data analysis, HistFitter \cite{Baak:2014wma}.
The observed and expected 95\% CL upper limits on the allowed cross-sections are shown in Fig.~\ref{fig:limits}.
For top squarks with decays into two light-quarks, the expected limit goes from 100 to 450~\GeV, 
while the observed limit excluding masses between 100 and 410~\GeV.\
If the decay is into a $b$-quark and a light-quark, masses between 100 and 550~\GeV{} are expected to be excluded,
with an observed exclusion going from 100 to 650~\GeV.
For scalar octet states




\begin{figure}
  \centering
  \subfloat[Inclusive selection]{\includegraphics[width=0.49\textwidth]{figuresINT2017/UpperCrossSections_RPVUDD_2sigmaInc}\label{subfig:limits_inc}}
  \subfloat[Two-tag selection]{\includegraphics[width=0.49\textwidth]{figuresINT2017/UpperCrossSections_RPVUDD_2sigma2B}\label{subfig:limits_twotag}}\\
  \subfloat[Two-tag selection]{\includegraphics[width=0.49\textwidth]{figuresINT2017/UpperCrossSections_RPVUDD_2sigmaColoron}\label{subfig:limits_twotag}}\\
  \caption{\label{fig:limits} Expected 95\% CL upper limit on the $\sigma\times BR$,
    compared to the theoretical cross-section for the direct pair-production of the different resonances considered in the search.
    The dashed black and solid red lines show the 95\% CL expected and observed limits respectively,
    including all uncertainties except the theoretical signal cross-section uncertainty.
    The solid yellow (green) band around the expected limit show the one (two) sigma uncertainties around this limit.
    The shaded colored cross-section band indicates the $\pm1\sigma$ variations due to theoretical uncertainties
    on the signal production cross-section given by renormalisation and factorisation scale and PDF uncertainties.}
\end{figure}


==> acknowledgements/Acknowledgements-main.tex <==
%\documentclass[11pt,a4paper]{article}
% Test document for ATLAS standard Acknowledgements.

\usepackage[backend=biber]{biblatex}

\PassOptionsToPackage{hyphens}{url}
\usepackage{hyperref}
\hypersetup{pdftitle={ATLAS Document}, pdfauthor={ATLAS Collaboration}} 
\hypersetup{colorlinks, breaklinks}
\hypersetup{linkcolor=blue, citecolor=blue, filecolor=black, urlcolor=blue}

\addbibresource{Acknowledgements.bib}

\begin{document}

\section*{Acknowledgements}

\input{Acknowledgements}

\printbibliography

\end{document}


